A Higher Radix Architecture for Quantum Carry-lookahead Adder

In this paper, we propose an efficient quantum carry-lookahead adder based on the higher radix structure. For the addition of two $n$-bit numbers, our adder uses $O(n)-O(\frac{n}{r})$ qubits and $O(n)+O(\frac{n}{r})$ T gates to get the correct answer in T-depth $O(r)+O(\log{\frac{n}{r}})$, where $r$ is the radix. Quantum carry-lookahead adder has already attracted some attention because of its low T-depth. Our work further reduces the overall cost by introducing a higher radix layer. By analyzing the performance in T-depth, T-count, and qubit count, it is shown that the proposed adder is superior to existing quantum carry-lookahead adders. Even compared to the Draper out-of-place adder which is very compact and efficient, our adder is still better in terms of T-count.

==> document/2-1-timeline.tex <==
%%%%%%%%%%timeline

\begin{tikzpicture}[
  man0/.style={rectangle,draw,fill=gray!10},  man1/.style={rectangle,draw,fill=cyan!15},  man2/.style={rectangle,draw,fill= yellow!26},%yellow!26 cyan
  woman/.style={rectangle,draw,fill=green!10,rounded corners=.8ex},
  grandchild/.style={grow=down,xshift=1em,anchor=west,
    edge from parent path={(\tikzparentnode.south) |- (\tikzchildnode.west)}},
  first/.style={level distance=4.6ex},
  second/.style={level distance=9.2ex},
  third/.style={level distance=13.8ex},
  first1/.style={level distance=4.6ex},
  second1/.style={level distance=23ex},
  third1/.style={level distance=42ex},
  level 1/.style={sibling distance=12em}]
    % Parents
    \coordinate
    %node[woman,anchor=center]{Jane}
    child[grow=up] {node[man0,anchor=center]{\large{Adders}}}
      % child[grow=right] {node[woman,anchor=west]{Jane}}
      %child[grow=down,level distance=0ex]
    [edge from parent fork down]
    % Children and grandchildren
    child{node[man1] {Quantum adders}
      child[grandchild,first1] {node[man2]{RCA}
      child[grandchild,first] {node[woman]{VBE\cite{VBE}}}
      child[grandchild,second] {node[woman]{Cuccaro \cite{Cuccaro}}}
      child[grandchild,third] {node[woman]{Takahashi \cite{Takahashi09}}}
      }
    child[grandchild,second1] {node[man2]{CLA}
      child[grandchild,first] {node[woman]{Draper Out-of-place \& In-place \cite{Draper08}}}
      child[grandchild,second] {node[woman]{Takahashi Adder \cite{Takahashi08} }}
      child[grandchild,third] {node[woman]{Takahashi CLA \cite{Takahashi09} }}
      }
    child[grandchild,third1] {node[man2]{Combination}
      child[grandchild,first] {node[woman]{Takahashi Combination \cite{Takahashi09} }}
      % child[grandchild,second]{node[woman]{......}}
      }}
    child{node[man1] {Unique quantum structure}
      child[grandchild,first] {node[woman]{Logical-And \cite{Craig_Gidney_2017}}}}
    child {node[man1] {Classical Adders}
      child[grandchild,first] {node[woman]{ MCC adder \cite{MCC1988}}}
      child[grandchild,second] {node[woman]{
      Higher radix adder\cite{classic_higher_radix}}}
    }
\end{tikzpicture}

